Automating the Last-Mile for High Performance Dense Linear Algebra

High performance dense linear algebra (DLA) libraries often rely on a general matrix multiply (Gemm) kernel that is implemented using assembly or with vector intrinsics. In particular, the real-valued Gemm kernels provide the overwhelming fraction of performance for the complex-valued Gemm kernels, along with the entire level-3 BLAS and many of the real and complex LAPACK routines. Thus,achieving high performance for the Gemm kernel translates into a high performance linear algebra stack above this kernel. However, it is a monumental task for a domain expert to manually implement the kernel for every library-supported architecture. This leads to the belief that the craft of a Gemm kernel is more dark art than science. It is this premise that drives the popularity of autotuning with code generation in the domain of DLA. This paper, instead, focuses on an analytical approach to code generation of the Gemm kernel for different architecture, in order to shed light on the details or voo-doo required for implementing a high performance Gemm kernel. We distill the implementation of the kernel into an even smaller kernel, an outer-product, and analytically determine how available SIMD instructions can be used to compute the outer-product efficiently. We codify this approach into a system to automatically generate a high performance SIMD implementation of the Gemm kernel. Experimental results demonstrate that our approach yields generated kernels with performance that is competitive with kernels implemented manually or using empirical search.

==> Makefile <==
all:
	pdflatex article.tex
	bibtex article
	pdflatex article.tex
	pdflatex article.tex

	gs \
 -sOutputFile=output.pdf \
 -sDEVICE=pdfwrite \
 -sColorConversionStrategy=Gray \
 -dProcessColorModel=/DeviceGray \
 -dCompatibilityLevel=1.4 \
 -dNOPAUSE \
 -dBATCH \
 article.pdf

package:
	tar czvf automating_last_mile_gemm.tar.gz ACM-Reference-Format-Journals.bst article.bbl *.tex queue.pdf BLIS_micro_kernel.png acmcopyright.sty acmsmall.cls Makefile biblio.bib analysis_plots/*.pdf figures/*.pdf

clean:
	rm -f *~ *.aux *.idx *.log *.blg *.bbl *.toc */*~ *.dvi *.lot *.out article.pdf article.ps *.ilg *.loa *.lof Results/*.aux



==> fig_queues.tex <==
\begin{center}
\begin{tikzpicture}
\node at (0, 0)[shape=rectangle, draw]{};
\node at (1, 0)[shape=circle, draw]{};

\node at (0, 0)[shape=rectangle, draw]{};
\node at (1, 0)[shape=circle, draw]{};

\node at (0, 1)[shape=rectangle, draw]{};
\node at (1, 1)[shape=circle, draw]{PERM/SHUF};

\node at (0, 2)[shape=rectangle, draw]{};
\node at (0.25, 2)[shape=rectangle, draw]{};
\node at (0.5, 2)[shape=rectangle, draw]{};
\node at (0.75, 2)[shape=rectangle, draw]{};
\node at (1, 2)[shape=rectangle, draw]{};

\node at (1, 2.5)[shape=circle, anchor=north west, draw]{ADD};

\node at (0, 3)[shape=rectangle, draw]{};
\node at (1, 3)[shape=circle, draw]{MUL};

\node at (0, 4)[shape=rectangle, draw]{};
\node at (1, 4)[shape=circle, draw]{LD//STO};
\end{tikzpicture}
\end{center}

==> mmm_prefetch.tex <==
\labday{ Wednesday April 29 2015 }



\experiment{Prefetching for MMM}

Let $N_p$ be the number of prefetch instructions that we issue per
$k_u$ unrolled outer products. Then we can find $N_p$ using the following
formula.

\begin{equation}
N_p = \frac{\frac{l}{8}}{m_r}
\end{equation}

Let $L_{LLC\rightarrow reg}$ and $L_{L2 \rightarrow reg}$ be the latency from
LLC to register and L2 to register respectively. Then the Latency from LLC to
L2 is defined as $L_{LLC\rightarrow L2} =L_{LLC\rightarrow reg} - L_{L2 \rightarrow reg}$.

Let $L_p$ be the latency in cycles from when the prefetch instruction is
issued and when the requested cache line reaches the L2 cache.Then $L_p =
L_{LLC\rightarrow L2} + L_{pref}$ where $L_{pref}$ is the latency between when
the prefetch instruction is decoded and when the read request hits the L3.



We know the number of prefetch instructions we need to issue now we need to
determine how far ahead to issue the prefetch. The idea is we determine how
many outer products will cover the latency of $L_p$ and that is our
distance. If $R$ is our rate of floating point computation per cycle and $l$
is our cache line size in bytes. Then we can find our distance (in terms of
number of cache lines) that we have to prefetch in order to have a timely
arrival of our data in L2.


\begin{equation}
\begin{array}{lcl}
D &=& \ceil{\frac{L_p}{L}} \\
L &=& \frac{2n_r\frac{l}{8}}{R}
\end{array}
\end{equation}



==> new_overview.tex <==
\begin{lstlisting}
  0. GOAL: High performance expert-tuned kernels for matrix-matrix multiply
  can be automated.

  1. Contribution
  - Reduce current problem to outer product
  - Model the relevant pieces of the problem (what we had reserved for
  experts)
  - automate the implementation (code generation and optimization)
  - Extending beyond matmul

  2. Why this matter
  - Last leg of automation for matmul, light at the end of the tunnel for the
  systematic reduction to high performance
  - experts don't always get it right
  - Extensible matmul like kernels
  -- Genomics
  -- Graph Analytics
  -- Machine Learning


  3. Hypothesis Testing
  + The Models
  -- are we picking the best instruction mix
  -- are we blocking appropriately
  -- are we scheduling efficiently
  -- are we prefetching correctly

  + uArch details
  -- Decoding Matters
  -- Minimal Loops
  -- Register coloring
  -- address modes mater

  + Comparison cross Machins
  -- Kerns vs ATLAS: they don't fully generate, and on wrong premise
  -- Kerns vs OpenBLAS/MKL/ACML: experts have blind-spots, hard to keep up
  -- Kerns vs Compilers [PoCC, icc on outer product]: hard problem to
  optimize, need the right mix of optimizations

  + Going Beyond
  -- parallel/hyperthreads (hit point)
  -- Floyd-Warshall - Graph analytics
  -- Linkage Disequillibrium - genomics
  -- KNN - machine learning


  Intro
  Model/Theory
  Mechanism
  Evaluation
  Summary
\end{lstlisting}

\section{The Operation}
.. reduce to outer product

\begin{lstlisting}
  ++ HP Mat Mul is a layering of loops to shuttle data to a tuned kernel
  -- goto/blis deconstruction
  -- Micro kernel

  Our contribution
  -- Micro kernel can be decomposed as an outer product
  -- Further we can permute our outer product. We are not restricted to an
  outer product.
  $ C = P_aab^tP_b$
  $ C = P_a^T(\Sigma_{p}^k (P_aa_p) (b^T_pP_b))P_b^T$...check
  -- We can break this outer product into several constituents
  -- Given an architecture there is an incredibly large search space: all the
  ways to splat, all the ways to load, all of the ways to accumulate
  -- If the combination of these constituents can be efficient then we can
  have an efficient
  ** Question, how do we find a mix of instructions for these parts that can
  sustain a high throughput?
\end{lstlisting}

\section{The Algorithm}
.. select the instruction mix for the outer product

\begin{lstlisting}
  ++ Our pipeline:
  -- have outer product dimensions (mr nr)
  -- determine instruction mix for our hardware that maximizes throughput
  (main: worry about bandwidth, lesser: worry about sub-blocking)
  -- implement that mix efficiently (main: worry about latency, lesser: worry
  about resources)

  ## Right no we focus on the instruction mix

  ++ We want to implement the outer-product with the set of instructions that
  maximizes throughput (according to our hardware model)
  -- This implementation will vary between different architectures because the
  throughput and latency of an instruction varies between architectures
  -- We need a mix of instructions that performs well
  -- If the outer product needs to be further reduced to several outer
  products that are implemented differently, but sustain a high throughput we
  take advantage of that.
  ** Show an example of an outer product implementation


  ++ How we do this: we enumerate all possible permuted outer products that
  can be implemented using a given ISA (with some restrictions), we then
  enumerate all tilings of these instruction based outer products that can
  implement our desired  Outer Product Kernel.
  -- We use a model of the hardware and queueing theory to estimate each
  possible tiling for the Outer Product Kernel.

  ++ Queueing theory throughput model
  -- Rather than implementing every kernel and timing...
  -- The queueing theory model allows us to estimate the steady-state
  throughput of many iterations of the outer product kernel. as we would see
  in the microkernel
  -- The model works as follows: we treat resources as queues, the
  instructions as tasks, and we use little's law to determine what our
  throughput would be given a mix of instructions. In the case where an
  instruction can go to multiple queues we split the tasks proportionally
  based on how much work is in the queue.
  -- This approach would allow us to do a backtrack based search for the best
  instruction mix combination.

  ++ System Implementation details:
  -- In general, broadcast and butterfly cover most hardware targets well
  -- For those we can cast the problem as the n-rooks problem for the
  permutation
  -- For more elaborate architectures we need a branch-and-bound approach
  -- Our current approach behaves as follows: Given an ISA We enumerate all
  possible permuted outer products, where A is simply loaded as a vector, and
  the B elements are allowed to be permuted. we also restrict to single
  load-type instruction for A and for B in order to get the smallest possible
  permuted outer products (see figure). 

  We fix the retrieval of the A
  elements to be loads, 
\end{lstlisting}

\section{The implementation }

We start with the dimension for $m_r,n_r,k_b,k_u$, but we have also included
register blocking dimensions $m_s,n_s$ so we can effectively schedule without
spilling. For the implementation, we can split it into three phases,
initialize, compute and finalize. We can perform some basic code motion such
that we minimize the number of loads by storing them into registers.


\subsection{Concept in C generating the code}

\begin{verbatim}
for( int pp = 0; pp < k_b; pp++ )
 for( int i = 0; i <  m_r; i ++ )
  for( int j = 0; j <  n_r; j ++ )
   for( int ii = i; ii <  i+m_s; ii ++ )
    for( int jj = j; jj < j+n_s; jj ++ )
      C[(ii,jj)] +=  A[(ii,pp)] * B[(pp,jj)];
\end{verbatim}


Splitting into phases:
\begin{verbatim}
for( int i = 0; i <  m_r; i ++ )
 for( int j = 0; j <  n_r; j ++ )
  for( int ii = i; ii < i+m_s; ii ++ )
   for( int jj = j; jj < j+n_s; jj ++ )
    c_reg[ii][jj] =  0;

for( int pp = 0; pp < k_b; pp++ )
 for( int i = 0; i <  m_r; i ++ )
  for( int j = 0; j <  n_r; j ++ )
   for( int ii = i; ii < i+m_s; ii ++ )
    for( int jj = j; jj < j+n_s; jj ++ )
     c_reg[ii][jj] +=  A[(ii,pp)] * B[(pp,jj)];

for( int i = 0; i <  m_r; i ++ )
 for( int j = 0; j <  n_r; j ++ )
  for( int ii = i; ii < i+m_s; ii ++ )
   for( int jj = j; jj < j+n_s; jj ++ )
    C[(ii,jj)] +=  c_reg[ii][jj];
\end{verbatim}


Now we focus on the computation phase and we take advantage of the fact that
we can reuse elements.
\begin{verbatim}
for( int pp = 0; pp < k_b; pp++ )
 for( int i = 0; i <  m_r; i ++ )
  for( int j = 0; j <  n_r; j ++ )
   for( int ii = i; ii < i+m_s; ii ++ )
    a_reg[ii] = A[ii+pp*m_r ];
    for( int jj = j; jj < j+n_s; jj ++ )
     b_reg[jj]      = B[jj+pp*n_r ];
     c_reg[ii][jj] +=  a_reg[ii] * b_reg[jj]
\end{verbatim}

We can split the computation up into the key components that we get from the
user. (implementation) Inside the code generator, the registers are treated as
a table with the 3 corresponding dimensions. The user defined instruction mix
is encoded in these functions.


\begin{verbatim}

inline void get_a_element( a_reg[][], A, ii, jj )
  a_reg[ii] = A[ ii+pp*m_r ];

inline void get_b_element( b_reg[][], B, ii, jj )
  b_reg[jj] = B[jj+pp*n_r ];

inline void compute( c_reg, a_reg, b_reg, C, A, B, ii,jj,pp )
 c_reg[ii][jj] +=  a_reg[ii] * b_reg[jj]

 // Initialize a_reg and b_reg as a table in space
 // Initialize c_reg as a table in space/time

for( int pp = 0; pp < k_b; pp++ )
 for( int i = 0; i <  m_r; i ++ )
  for( int j = 0; j <  n_r; j ++ )
   for( int ii = i; ii < i+m_s; ii ++ )
    get_a_element(a_reg, ii,j );
    for( int jj = j; jj < j+n_s; jj ++ )
     compute( c_reg, a_reg, b_reg, C, A, B, ii,jj,pp )


     get_a ---> dup so input is mxk = 1x4 output is 1x4
     get_b ---> vload so input is kxn = 1x4 output is 1x4
     compute -> fma input is mxn 1x4        output is 1x4
\end{verbatim}


These functions have their own dimensions. For example each call of the
$\texttt{get\_a\_element}$ function has an input of $R^{1 \times v}$ where $v$ is
our vector length. Similarly, each call of $\texttt{get\_b\_element}$ and
$\texttt{compute}$ are $1 \times ... $.

The key insight is that user has given us our register blocking dimensions
$m_r$ and $n_r$  and our register partitions $m_s$ and $n_s$, along with the
instruction mixes encoded as these helper functions for retrieving $A$ and $B$
and computing.

For example, if $m_s\times n_s = 4\times 4 $ and we are applying the butterfly
permutations to $B$, then conceptually we would encode that instruction mix as
follows:


\begin{verbatim}
  void get_b_element( b_reg[][], B, ii, jj )
  {
    if( jj mod v == 0 )
    switch( jj )
    {
      case 0:
      b_reg[jj] = vload( &B[jj] )
      case 1:
      b_reg[jj] = shuffle( b_reg[jj-1] )
      case 2:
      b_reg[jj] = permute( b_reg[jj-1] )
      case 2:
      b_reg[jj] = shuffle( b_reg[jj-1] )
    }
  }
\end{verbatim}

Note, that we are not actually implementing this function and its associated
overhead, we are simply capturing the instruction mix. This function is
encoded in python and the code generator uses this to determine the required
operations and their dependencies. What we really have is:

\begin{verbatim}

  def get_b_element( var array b_reg[][], ptr B, ii, jj )
   options = { 0: assign( b_reg[jj], vload(B,jj)),
               1: assign( b_reg[jj], shuffle(b_reg[jj-1]) ),
               2: assign( b_reg[jj], permute(b_reg[jj-1]) ),
               3: assign( b_reg[jj], shuffle(b_reg[jj-1]) )}
   if ii mod v = 0
    return options[jj]

\end{verbatim}

This python based function allows the user to pass their desired instruction
mix to the code generator. The generator uses this 


This can be further extended
  
\begin{verbatim}
  assign( reg_xx, operation) // creates new node

  operation --> has constraints to it for OASIC
\end{verbatim}









%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{verbatim}
for( int pp = 0; pp < k_b; pp++ )
 for( int ii = 0; ii <  m_r; ii ++ )
  for( int jj = 0; jj <  n_r; jj ++ )
    C[(ii,jj)] +=  A[(ii,pp)] * B[(pp,jj)];
\end{verbatim}


\begin{verbatim}
for( int pp = 0; pp < k_b; pp++ )
 for( int ii = 0; ii <  m_r; ii ++ )
  for( int jj = 0; jj <  n_r; jj ++ )
    C[(ii,jj)] +=  A[ii+pp*m_r ] * B[jj+pp*n_r];
\end{verbatim}


Split operation into 3 phases centered around a block of temporary C
registers. First initialize the temporaries, then perform the computation,
finally write back the result. 

\begin{verbatim}

for( int ii = 0; ii <  m_r; ii ++ )
 for( int jj = 0; jj <  n_r; jj ++ )
  c_reg[ii][jj] =  0;


for( int pp = 0; pp < k_b; pp++ )
 for( int ii = 0; ii <  m_r; ii ++ )
  for( int jj = 0; jj <  n_r; jj ++ )
    c_reg[ii][jj] +=  A[ii+pp*m_r ] * B[jj+pp*n_r];


for( int ii = 0; ii <  m_r; ii ++ )
 for( int jj = 0; jj <  n_r; jj ++ )
   C[(ii,jj)] +=  c_reg[ii][jj];

\end{verbatim}




\begin{verbatim}
..
\end{verbatim}


We can perform some basic code motion.
\begin{verbatim}

for( int ii = 0; ii <  m_r; ii ++ )
 for( int jj = 0; jj <  n_r; jj ++ )
  c_reg[ii][jj] =  0;


for( int pp = 0; pp < k_b; pp++ )
 for( int ii = 0; ii <  m_r; ii ++ )
  a_reg[ii] = A[ii+pp*m_r ];
  for( int jj = 0; jj <  n_r; jj ++ )
   b_reg[jj] = B[jj+pp*n_];
   c_reg[ii][jj] +=  a_reg[ii] * b_reg[jj];


for( int ii = 0; ii <  m_r; ii ++ )
 for( int jj = 0; jj <  n_r; jj ++ )
   C[(ii,jj)] +=  c_reg[ii][jj];

\end{verbatim}

Here we can perform some memory addressing optimization that are fairly
portable.

\begin{verbatim}
OFFSET = 128B // We center the addresses at the middle of the instructions range

ptr *A_ptr = &A - OFFSET;
ptr *B_ptr = &B - OFFSET;

for( int ii = 0; ii <  m_r; ii ++ )
 for( int jj = 0; jj <  n_r; jj ++ )
  c_reg[ii][jj] =  0;


for( int p = 0; p < k_b; p+= k_u )
A_ptr += k_u*m_r;
B_ptr += k_u*n_r;
#unroll
#swp
for( int pp = 0; pp < k_u; pp++ )
  for( int ii = 0; ii <  m_r; ii ++ )
  a_reg[ii] = A_ptr[ii+pp*m_r + OFFSET ];
   #vector
   for( int jj = 0; jj <  n_r; jj ++ )
    b_reg[jj] = B_ptr[jj+pp*n_ + OFFSET ];
    c_reg[ii][jj] +=  a_reg[ii] * b_reg[jj];


for( int ii = 0; ii <  m_r; ii ++ )
 for( int jj = 0; jj <  n_r; jj ++ )
   C[(ii,jj)] +=  c_reg[ii][jj];

\end{verbatim}




